Effective and Scalable Clustering on Massive Attributed Graphs

Given a graph G where each node is associated with a set of attributes, and a parameter k specifying the number of output clusters, k-attributed graph clustering (k-AGC) groups nodes in G into k disjoint clusters, such that nodes within the same cluster share similar topological and attribute characteristics, while those in different clusters are dissimilar. This problem is challenging on massive graphs, e.g., with millions of nodes and billions of edges. For such graphs, existing solutions either incur prohibitively high costs, or produce clustering results with compromised quality. In this paper, we propose ACMin, an effective approach to k-AGC that yields high-quality clusters with cost linear to the size of the input graph G. The main contributions of ACMin are twofold: (i) a novel formulation of the k-AGC problem based on an attributed multi-hop conductance quality measure custom-made for this problem setting, which effectively captures cluster coherence in terms of both topological proximities and attribute similarities, and (ii) a linear-time optimization solver that obtains high-quality clusters iteratively, based on efficient matrix operations such as orthogonal iterations, an alternative optimization approach, as well as an initialization technique that significantly speeds up the convergence of ACMin in practice. Extensive experiments, comparing 11 competitors on 6 real datasets, demonstrate that ACMin consistently outperforms all competitors in terms of result quality measured against ground-truth labels, while being up to orders of magnitude faster. In particular, on the Microsoft Academic Knowledge Graph dataset with 265.2 million edges and 1.1 billion attribute values, ACMin outputs high-quality results for 5-AGC within 1.68 hours using a single CPU core, while none of the 11 competitors finish within 3 days.

==> algo.tex <==
\section{A First-Cut Solution}\label{sec:acmc}
\begin{algorithm}[!t]
\begin{small}
	\caption{\asc}
	\label{alg:asc}
	\KwIn{$G, k, t_e, t_m,\alpha,\beta$.}
	\KwOut{$\YM^{\prime}$.}
	Compute $\PaM$ by Equation \eqref{eq:pam}\;
	$\SM_0 \gets \IM,\ t\gets \frac{1}{\alpha}$\;
    \lFor{$\ell\gets 1$ to $t$}{
        $\SM_\ell \gets (1-\alpha)\cdot((1-\beta)\cdot\PtM+\beta\cdot \PaM)\cdot \SM_{\ell-1}+\SM_0$
    }
    $\SM \gets \alpha\cdot \SM_t$\;
    % $\FM_0 \gets \mathsf{InitCluster}(\PtM,\alpha,K)$\;
    % $\YM^{\prime} \gets \mathsf{InitNCI}(\PtM, \alpha, K)$\;
    % $\FM_0 \gets (\YM^{\prime}\YM^{\prime\top})^{-\frac{1}{2}}\YM^{\prime}$\;
    $\FM \gets$ the top-$k$ eigenvectors of $\SM$ with $t_e$ iterations\;
    $\YM \gets k\textrm{-}\mathsf{Means}(\FM, t_m)$\;
	\Return $\YM$\;
\end{small}
\end{algorithm}

A straightforward solution is to use XXX...
However, 


===

In this section, we first introduce the classic $\mathsf{USC}$ method (\ie {\em unormalized spectral clustering} \cite{von2007tutorial}) and how to adopt it as a first-cut solution to solve the ACMin problem. We then further analyse the ineffectiveness and inefficiency of \asc in Section \ref{sec:asc-analysis} and \ref{sec:asc-time} respectively.

Algorithm \ref{alg:asc} outlines the pseudo-code of \asc. Given an attributed input graph $G$, the number $k$ of clusters, the numbers $t,t_e,t_m$ of iterations, and the random walk factors $\alpha,\beta$ as inputs, \asc runs with two phases: (i) finding top-$k$ eigenvectors $\FM$ of the attributed random walk matrix $\SM$ (Lines 1-5); and (ii) generating an NCI $\YM$ via \kmeans with $\FM$ (Line 6). It is easy to verify that Lines 1-4 in Algorithm \ref{alg:asc} return exact attributed random walk matrix $\SM$. At Lines 5-6, \asc finds the top-$k$ eigenvectors $\FM$ of $\SM$ as a rough solution. Particularly, $\FM$ is referred to as the top-$k$ eigenvectors of $\SM$ if their corresponding eigenvalues are the $k$ largest. 
% In the following, we detail how Lines 5-6 in Algorithm \ref{alg:asc} yields an approximate solution to the ACMin problem. \asc relaxes the constraint on node-cluster indicator $\YM$ (\ie $\YM\in \mathbb{1}^{k\times n}$) such that each entry $\YM[c_i,v_j]$ can take real values but ensure $\FM\FM^{\top}=\IM$ where $\FM=(\YM\YM^{\top})^{-\frac{1}{2}} \YM$. Then, Eq. \eqref{eq:objt} is transformed into a new objective function as follows:
% Theorem \ref{thrm:topk-eigen} indicates that solving the objective function in Equation~\eqref{eq:objr} is to find the top-$k$ eigenvectors $\FM$ of $\SM$.
After obtaining $\FM$, Algorithm \ref{alg:asc} invokes \kmeans with the top-$k$ eigenvectors $\FM$ and the number of iterations $t_m$ as inputs to obtain an NCI $\YM$ (Line 6), and finally returns $\YM$ as the clusterization result (Line 7).

% To solve Eq. \eqref{eq:objr}, we add Lagrange multipliers to incorporate the constraints on $\FM$ and render the partial derivatives with respect to $\FM[c_i]$ to zero. Then, we have
% \begin{equation*}
% \textstyle \frac{\partial}{\partial\  \FM[c_i]}\left(\sum_{i=1}^{k}{\FM[c_i](\IM-\SM)\FM[c_i]^{\top}+\sum_{i=1}^{k}{\overline{\zeta}_i(1-\FM[c_i]\cdot\FM[c_i]^{\top})}}\right)=0,
% \end{equation*}
% and thus $(\IM-\SM)\cdot\FM[c_i]^{\top}=\overline{\zeta}_i\cdot\FM[c_i]^{\top}$, which implies that $(1-\overline{\zeta}_i,\FM[c_i])$ is an eigenpair of $\SM$. Let $\zeta_i=1-\overline{\zeta_i}$. Eq. \eqref{eq:objr} is equivalent to finding $k$ eigenvectors $\FM$ of $\SM$ such that their corresponding eigenvalues $\zeta_1,\zeta_2,\cdots,\zeta_k$ maximize $\sum_{i=1}^{k}{\zeta_i}$.
% Note that minimizing Eq. \eqref{eq:objr} is no longer NP-hard and the optimal $\Psi^{\prime}(\FM)$ is always no greater than the optimal $\Psi(\YM)$, \ie $\Psi^{\prime}(\FM) \le \phi^*$. 
% Additionally, by Lemma \ref{lem:stsum}, $\sum_{v_j\in V}{\SM[v_i,v_j]}=1-(1-\alpha)^{t+1}\ \forall{v_i\in V}$. 
% \begin{lemma}[\cite{haveliwala2003second}]\label{lem:stoch-eigen}
% Given a $\mathbf{M}\in \mathbb{R}^{n\times n}$ satisfying $\sum_{j=1}^{n}{\mathbf{M}[i,j]}=1\ \forall{1\le i\le n}$ and each entry $\mathbf{M}[i,j]\ge 0\ \forall{1\le i,j\le n}$, the largest eigenvalue $\lambda_1$ of $\mathbf{M}$ is 1.
% \end{lemma}
% Consequently, according to Lemma \ref{lem:stoch-eigen}, the largest eigenvalue $\lambda_1$ of $\SM$ is $1-(1-\alpha)^{t+1}$ and its corresponding eigenvector is $[n^{-\frac{1}{2}},n^{-\frac{1}{2}},\cdots,n^{-\frac{1}{2}}]$, which is useless for determining clusters. Instead, to maximize $\sum_{i=1}^{k}{\zeta_i}$, we choose $\zeta_1=\lambda_{2},\zeta_2=\lambda_{3},\cdots,\zeta_k=\lambda_{k+1}$ where $\lambda_{2},\lambda_{2},\cdots,\lambda_{k+1}$ are the second-$(k+1)$-th largest eigenvalues of $\SM$. As a result, $\FM$ is the $k$ eigenvectors of $\SM$ corresponding to $\lambda_{2},\lambda_{2},\cdots,\lambda_{k+1}$, unless otherwise specified, which is referred to as the top-$k$ eigenvectors of $\SM$ in this paper. To put it simply, solving the objective function in Equation~\eqref{eq:objr} is to find the top-$k$ eigenvectors $\FM$ of $\SM$. 


\subsection{Correctness Analysis of \asc}\label{sec:asc-analysis} 
% The basic idea of \asc is relaxing the constraint on the NCI $\YM$ (\ie $\YM\in \mathbb{1}^{k\times n}$) such that each entry $\YM[c_i,v_j]$ can take real values but ensure $\FM\FM^{\top}=\IM$ where $\FM=(\YM\YM^{\top})^{-\frac{1}{2}} \YM$, and then 
% Finding the top-$k$ eigenvectors $\FM$ of $\SM$ in \asc is actually to find the optimal $\FM$ to Eq. \eqref{eq:objr} (see Theorem \ref{thrm:topk-eigen} for more details).
% \begin{equation}\label{eq:objr}
% \min_{\FM\in\mathbb{R}^{k\times n}, \FM\FM^{\top}=\IM}{\Psi^{\prime}(\FM)=\frac{2}{k}\cdot\textrm{trace}(\FM\cdot(\IM-\SM)\cdot\FM^{\top})}.
% \end{equation}
As introduced, \asc derives an NCI $\YM$ from $\FM$ via \kmeans. % Theorem \ref{thrm:topk-eigen} indicates that solving the objective function in Equation~\eqref{eq:objr} is to find the top-$k$ eigenvectors $\FM$ of $\SM$.
Specifically, given a $k\times n$ matrix $\FM$, mathematically, \kmeans finds $k$ disjoint clusters $C_1,C_2,\cdots,C_k$ of $G$ such that
\begin{equation*}
\textstyle \min_{C_1,C_2,\cdots,C_k}{\sum_{i=1}^{k}{\sum_{v_j\in C_i}{\lnorm{\FM[:,v_j]-\frac{1}{|C_i|}\sum_{v_l\in C_i}{\FM[:,v_l]}}^2_2}}},
\end{equation*}
which can be rewritten as an NCI-based matrix form, \ie
% \begin{equation}\label{eq:kmeans}
% \min_{\YM\in \mathbb{1}^{k\times n},\XM\in \mathbb{R}^{k\times k}}{\lnorm{\FM-\XM\YM}^2_F}.
% \end{equation}
\begin{align}
&\textstyle \min_{\YM\in \mathbb{1}^{k\times n}}{\lnorm{\FM^{\top}-\YM^{\top}\XM}^2_F}\label{eq:kmeans},\\
&\textstyle \textrm{where}\ \XM=(\YM\YM^{\top})^{-1}\YM\FM^{\top}\label{eq:kmx}.
\end{align}
\kmeans solves Eq. \eqref{eq:kmeans}  by using the expectation-maximization (EM) algorithm. Initially, it sets $\YM$ as a random incicator matrix (\ie $\mathbb{1}^{k\times n}$) and computes $\XM$ via Eq. \eqref{eq:kmx} accordingly. Then, with $\XM$ fixed, each entry $\YM[c_i,v_j]$ for cluster $C_i$ and node $v_j$ is updated as
\begin{equation*}
\textstyle \YM[c_i,v_j]=\begin{cases}
\textstyle 1, &\quad\text{$i=\argmin{1\le l\le k}{\lnorm{\FM[:,v_j]-\XM[l]}^2_2}$},\\
\textstyle 0, &\quad\text{else}.
\end{cases}
\end{equation*}
After that, with $\YM$ fixed, it recomputes $\XM$ by Eq. \eqref{eq:kmx} accordingly. \kmeans repeats the above optimization process in an alternative and iterative manner until convergence. Suppose that we find the optimal $\YM$ to Eq. \eqref{eq:kmeans}. Then we have $\FM=\FM\YM^{\top}(\YM\YM^{\top})^{-1}\YM$, which implies that \asc actually finds an NCI $\YM$ that minimizes the following objective function
\begin{align*}
&\textstyle \frac{2}{k}\cdot\textrm{trace}(\FM\YM^{\top}(\YM\YM^{\top})^{-1}\YM\cdot(\IM-\SM)\cdot(\FM\YM^{\top}(\YM\YM^{\top})^{-1}\YM)^{\top}),\\
&\textstyle\quad\quad\quad \textrm{where $\FM$ is the top-$k$ eigenvectors of $\SM$},
\end{align*}
which is totally different from our objective function in Eq. \eqref{eq:objt}. In a nutshell, the NCI $\YM$ returned by \asc fails to provide us an attributed conductance that approaches the optimal attributed conductance $\phi^{*}$ of $G$.

\subsection{Complexity Analysis}\label{sec:asc-time}

\asc mainly consists of three parts. First, considering that there are $|E_R|$ non-zero elements in $\RM$, computing $\PaM$ takes $O(|E_R|\cdot n)$ time. Second, the computation of $\SM$ involves $t=\frac{1}{\alpha}$ iterations of matrix multiplications with $\PtM$ and $\PaM$, both of which are stored as sparse matrices. Thus the time cost is $O(nt\cdot (|E_V|+nnz(\PaM)))$. Third, the top-$k$ eigendecomposition of $\SM$ requires $O(kt_e\cdot (|E_V|+nnz(\PaM)))$ time with $t_e$ iterations \cite{demmel1997applied}. For an $n\times k$ matrix $\FM^{\top}$, \kmeans runs in $O(nk^2t_m)$ time. Overall, the time complexity of \asc is $$\textstyle O\left((|E_V|+nnz(\PaM))\cdot (\frac{n}{\alpha}+kt_e)+nk^2t_m\right),$$
which equals $O(n^3)$ when $|\PaM|=n^2$, $k,\alpha,t_e$ and $t_m$ are regarded as constants. In addition, \asc requires the materialization of $\SM$. Therefore, the space complexity of \asc is $O(n^2+|E_R|)$.
